Predicting global usages of resources endowed with local policies

The effective usages of computational resources are a primary concern of up-to-date distributed applications. In this paper, we present a methodology to reason about resource usages (acquisition, release, revision, ...), and therefore the proposed approach enables to predict bad usages of resources. Keeping in mind the interplay between local and global information occurring in the application-resource interactions, we model resources as entities with local policies and global properties governing the overall interactions. Formally, our model takes the shape of an extension of pi-calculus with primitives to manage resources. We develop a Control Flow Analysis computing a static approximation of process behaviour and therefore of the resource usages.

==> VCPref-default.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Package `Vaucanson-G'  version 0.4
%%
%% This is file `VCPref-default'.
%%
%% IMPORTANT NOTICE:
%%
%% Copyright (C) 2002-2008 Sylvain Lombardy and Jacques Sakarovitch
%%
%% This package may be distributed under the terms of the LaTeX Project
%% Public License, as described in lppl.txt in the base LaTeX distribution.
%% Either version 1.0 or, at your option, any later version.
%%
%% DESCRIPTION:
%%
%%   `VCPref-default' contains default values for Vaucanson-G    
%%              
%%   Editing the file and changing these values is of course possible 
%%   but users are advised to rather edit the file `VCPref-mystyle' 
%%   instead.
%%   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scales  settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\LargeScale}{0.85}        %float : argument of a \scalebox
\renewcommand{\MediumScale}{0.6}        %float
\renewcommand{\SmallScale}{0.5}		%float
\renewcommand{\TinyScale}{0.42}		%float
\renewcommand{\VCGridScale}{1}  % scale of psunit (in cm)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% State geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\LargeStateDiameter}{1.2cm}     %length
\setlength{\MediumStateDiameter}{.9cm}	   %length
\setlength{\SmallStateDiameter}{.6cm}      %length
\setlength{\VerySmallStateDiameter}{.3cm}  %length
\renewcommand{\VSStateLineCoef}{.6}        %float: coef*\StateLineWidth
\renewcommand{\StateDimen}{outer}      		
\renewcommand{\StateDblDimen}{middle}	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% State drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetStateLineStyle{solid}		%% aspect (none, dashed, dotted)
\SetStateLineColor{black}		%% color
\SetStateLineWidth{1.8pt}		%% length
\SetStateFillStatus{solid}		%% aspect
\SetStateFillColor{white}		%% color
\renewcommand{\SmallStateFillStatus}{solid} %
\renewcommand{\SmallStateFillColor}{white} %
\SetStateLabelColor{black}		%% color
\SetStateLabelScale{1.7}		%% float
\FixStateLineDouble{0.6}{0.4}  %% Double style: \StateLineDblCoef, 
\StateLineDblfalse             %%   \StateLineDblSep, *\StateLineWidth
%%% Dimmed states
% LineStyle,LineColor,LineCoef (*\StateLineWidth),LabelColor,FillColor
\FixDimState{solid}{gray}{1}{gray}{white}  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Edge drawing  (Edge is understood here as transitions!)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetEdgeLineStyle{solid}                %% aspect
\SetEdgeLineColor{black}		%% color
\SetEdgeLineWidth{1pt}			%% length
\EdgeLineDblfalse 
% coefs*\EdgeLineWidth -> (width of lines, distance)
\FixEdgeLineDouble{0.5}{0.6}		%% 
\SetEdgeLabelColor{black}		%% color
\SetEdgeLabelScale{1.7}		        %% float
%%% arrows
\SetEdgeArrowWidth{5pt}		%width of the edge arrow
\SetEdgeArrowLengthCoef{1.4}    % 
\setlength{\EdgeDblArrowWidth}{5.5pt}  % width for double transitions
\renewcommand{\EdgeDblArrowLengthCoef}{1.7} 
\SetEdgeArrowInsetCoef{0.1}	%float : coef*\EdgeArrowWidth
\SetEdgeArrowStyle{->}	        %style (other styles : <-, |-|, -|,...)
\renewcommand{\EdgeRevArrowStyle}{<-}   %style for reverse transitions
%%% Dimmed edges
%  LineStyle,LineCoef,LineColor,LabelColor
\FixDimEdge{solid}{1.2}{gray}{gray}     %% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Edge geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetEdgeOffset{0pt}                     %% length
\renewcommand{\ForthBackEdgeOffset}{5}	%% coef*\EdgeLineWidth -> offset
\setlength{\EdgeNodeSep}{0pt}
% int,color : coef*\EdgeLineWidth -> width of border
\FixEdgeBorder{2}{white}		%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ZZ geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\ZZSize}{.9cm}		% length : apparent diameter
\renewcommand{\ZZShape}{0.5}		% coef: opening of the ZZ
\SetZZLineWidth{1.7}			% float
%  coef*\ZZSize -> distance added for labels
\renewcommand{\TransLabelZZCoef}{0.6}	% float 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Arc geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetArcAngle{15}			%% int (degree)
\SetLArcAngle{30}			%% int (degree)
\SetArcCurvature{0.8}			%% float
\SetArcOffset{1pt}			%% length
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Loop geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\LoopAngle}{30}
\renewcommand{\CLoopAngle}{22}
\renewcommand{\LoopVarAngle}{28}
\SetLoopOffset{0pt}			%% length
\setlength{\LoopVarOffset}{.7pt}
% loop curvature
\renewcommand{\LoopOnLargeState}{5.8} 		%float
\renewcommand{\LoopOnMediumState}{7}		%float  
\renewcommand{\LoopOnSmallState}{9.6} 		%float
\renewcommand{\LoopOnVariableState}{5.1}        %float
\renewcommand{\CLoopOnLargeState}{6}		%float
\renewcommand{\CLoopOnMediumState}{8}		%float
\renewcommand{\CLoopOnSmallState}{12}		%float
\renewcommand{\CLoopOnVariableState}{5.2}       %float
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge labels  positioning
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\TransLabelSep}{3.5pt}
%  per cent (use \Fix..LabelPosit with values in [10;90])
\renewcommand{\EdgeLabelPosit}{.45}   %
\renewcommand{\EdgeLabelRevPosit}{.55}
\renewcommand{\ArcLabelPosit}{.40}
\renewcommand{\ArcLabelRevPosit}{.60}
\renewcommand{\LArcLabelPosit}{.40}
\renewcommand{\LArcLabelRevPosit}{.60}
\renewcommand{\LoopLabelPosit}{.25}
\renewcommand{\LoopLabelRevPosit}{.75}
\renewcommand{\CLoopLabelPosit}{.25}
\renewcommand{\CLoopLabelRevPosit}{.75}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initial states parameters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  float : coef *\StateDiameter for size of initial and final arrows
\renewcommand{\ArrowOnMediumState}{1.5}		%float
\renewcommand{\ArrowOnSmallState}{1.7} 		%float
\renewcommand{\ArrowOnLargeState}{1.3}		%float
\renewcommand{\ArrowOnVerySmallState}{5} 	%float
%
\renewcommand{\InitStateLabelPosit}{.10}
\renewcommand{\InitStateLabelRevPosit}{.90}
\renewcommand{\FinalStateLabelPosit}{.90}
\renewcommand{\FinalStateLabelRevPosit}{.10}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initialization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetVCDirectory{}        %default dir=current dir
\HideFrame
\HideGrid
\MediumPicture
\HideName
\RigidLabel
\FullState				%% PlainState
\MediumState
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput


==> Vaucanson-G.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Package `VauCanSon-G'  version 0.4
%%
%% This is file `VauCanSon-G'.
%%
%% IMPORTANT NOTICE:
%%
%% Copyright (C) 2002-2008 Sylvain Lombardy and Jacques Sakarovitch
%%
%% This package may be distributed under the terms of the LaTeX Project
%% Public License, as described in lppl.txt in the base LaTeX distribution.
%% Either version 1.0 or, at your option, any later version.
%%
%% DESCRIPTION:
%%
%%   `VauCanSon-G' is the main file of the package and contains all 
%%   macro definitions file. 
%%  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Writing VauCanSon-G macro
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\VCSG}%
   {\textsc{V$\overline{\text{au}}$C%
    \raisebox{.3ex}{$\underline{\text{an}}$}S%
    $\overline{\text{on}}$-G}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Commands for geometric constructions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% constants 
\newcommand{\SQRTwo}{0.717}
\newcommand{\SQRThree}{1.732}
\newcommand{\GoldMean}{0.618}
\newcommand{\GoldMeanI}{1.618}
\newcommand{\SQRGoldMeanI}{1.272}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Edge label drawing macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Separator in compound labels (eg \IOL{input}{output})
\newcommand{\IOL}[2]{#1\!\mid\! #2}
%%% Stacked labels
\newcommand{\StackTwoLabels}[2]%
   {\renewcommand{\arraystretch}{0.75}%
    \begin{array}{c}#1\\ #2 \end{array}%
    \renewcommand{\arraystretch}{1.333}}
\newcommand{\StackThreeLabels}[3]%
   {\renewcommand{\arraystretch}{0.75}%
    \begin{array}{c}#1\\ #2 \\ #3 \end{array}%
    \renewcommand{\arraystretch}{1.333}}
%%% Stacked labels with +
\newcommand{\StackTwoLabelsP}[2]%
   {\renewcommand{\arraystretch}{0.75}%
    \begin{array}{c}#1\\ + \\ #2 \end{array}%
    \renewcommand{\arraystretch}{1.333}}
\newcommand{\StackThreeLabelsP}[3]%
   {\renewcommand{\arraystretch}{0.75}%
    \begin{array}{c}#1\\ + \\ #2 \\ + \\ #3 \end{array}% 
    \renewcommand{\arraystretch}{1.333}}
%%% Lined up labels (with +)
\newcommand{\LineTwoLabelsP}[2]{#1 + #2} 
\newcommand{\LineThreeLabelsP}[3]{#1 + #2 + #3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scales  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\LargeScale}{0.85}
\newcommand{\MediumScale}{0.6}
\newcommand{\SmallScale}{0.5}
\newcommand{\TinyScale}{0.42}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% State parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Size = StateDiameter
%%% The preset sizes are given in cm, and not in "psunits".
%%% This allows to use different scales for the whole figure 
%%% and for the "drawing grid".
\newlength{\MediumStateDiameter}
\newlength{\SmallStateDiameter}
\newlength{\LargeStateDiameter}
\newlength{\VerySmallStateDiameter}
\setlength{\MediumStateDiameter}{.9cm}
\setlength{\SmallStateDiameter}{.6cm}
\setlength{\LargeStateDiameter}{1.2cm}
\setlength{\VerySmallStateDiameter}{.3cm}
%%% Border line = StateLine
\newlength{\StateLineWidth}        % width
\setlength{\StateLineWidth}{1.8pt}
\newcommand{\StateLineStyle}{solid} % style
\newcommand{\StateLineColor}{black}
\newif\ifStateLineDbl \StateLineDblfalse 
\newcommand{\StateLineDblCoef}{0.6} 
\newcommand{\StateLineDblSep}{0.4} 
\newcommand{\VSStateLineCoef}{.6} % coef. for very small state
%%% State background and label
\newcommand{\StateFillStatus}{solid} 
\newcommand{\StateFillColor}{white}
\newcommand{\StateLabelColor}{black}
\newcommand{\StateLabelScale}{1.7}
\newcommand{\SmallStateFillStatus}{solid} %
\newcommand{\SmallStateFillColor}{white} %
   % As they have usually no labels it useful
   % to have a coloring facility for the "SmallState"
%%%  Dimmed states (e.g. for non accessible states)
\newcommand{\DimStateLineStyle}{solid} 
\newcommand{\DimStateLineCoef}{1} % 
\newcommand{\DimStateLineColor}{gray}
\newcommand{\DimStateLabelColor}{gray}
\newcommand{\DimStateFillColor}{white}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge drawing parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% line
\newlength{\EdgeLineWidth}
\setlength{\EdgeLineWidth}{1pt}
\newcommand{\EdgeLineStyle}{solid}
\newif\ifEdgeLineDbl \EdgeLineDblfalse 
%\newcommand{\EdgeLineDblStatus}{false} 
\newcommand{\EdgeLineDblCoef}{0.5} 
\newcommand{\EdgeLineDblSep}{0.6} 
\newcommand{\EdgeLineColor}{black}
% arrow
\newlength{\EdgeArrowWidth}
\setlength{\EdgeArrowWidth}{5pt}
\newlength{\EdgeDblArrowWidth}
\setlength{\EdgeDblArrowWidth}{5.5pt}
\newcommand{\EdgeArrowLengthCoef}{1.4}
\newcommand{\EdgeDblArrowLengthCoef}{1.7}
\newcommand{\EdgeArrowInset}{0.1}
\newcommand{\EdgeArrowStyle}{->}
\newcommand{\EdgeRevArrowStyle}{<-}
% border
\newcommand{\EdgeLineBorderCoef}{2}
\newcommand{\EdgeLineBorderColor}{white}
% label
\newcommand{\EdgeLabelColor}{black}
\newcommand{\EdgeLabelScale}{1.7}
%%% Dimmed edges 
\newcommand{\DimEdgeLineCoef}{1.2} 
\newcommand{\DimEdgeLineStyle}{solid} 
\newcommand{\DimEdgeLineColor}{gray}
\newcommand{\DimEdgeLabelColor}{gray}
%%% Zigzag edges parameter
\newlength{\ZZSize}
\setlength{\ZZSize}{.9cm} % =\MediumStateDiameter
\newcommand{\ZZShape}{0.5}
\newcommand{\ZZLineWidth}{1.7} % coefficient multiplicateur
%  coef*\ZZSize -> distance added for labels
\newcommand{\TransLabelZZCoef}{0.6} % 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge geometric parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Edge 
\newlength{\EdgeOffset}
\setlength{\EdgeOffset}{0pt}
\newcommand{\ForthBackEdgeOffset}{5}% coef
\newlength{\EdgeNodeSep}\setlength{\EdgeNodeSep}{0pt}
% Arc parameters
\newcommand{\VaucArcAngle}{15}
\newcommand{\VaucArcCurvature}{0.8}
\newlength{\VaucArcOffset}\setlength{\VaucArcOffset}{1pt}
% Large Arc parameters
\newcommand{\VaucLArcAngle}{30}
\newcommand{\VaucLArcCurvature}{0.8}
\newlength{\LoopOffset}\setlength{\LoopOffset}{0pt}
\newlength{\LoopVarOffset}\setlength{\LoopVarOffset}{.7pt}
\newcommand{\LoopAngle}{30}
\newcommand{\CLoopAngle}{22}
\newcommand{\LoopVarAngle}{28}
% Size of loops (depending on the size of the state)
\newcommand{\LoopOnMediumState}{7}
\newcommand{\LoopOnSmallState}{9.6} 
\newcommand{\LoopOnLargeState}{5.8} 
\newcommand{\LoopOnVariableState}{5.1} 
\newcommand{\LoopOnVerySmallState}{15} 
\newcommand{\CLoopOnMediumState}{8}
\newcommand{\CLoopOnSmallState}{12}
\newcommand{\CLoopOnLargeState}{6}
\newcommand{\CLoopOnVariableState}{5.2}
%\newcommand{\CLoopOnVerySmallState}{14} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Edge label parameters --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% label distance from transition
\newlength{\TransLabelSep}\setlength{\TransLabelSep}{3.5pt}
% label position on transitions
\newcommand{\EdgeLabelPosit}{.45}\newcommand{\EdgeLabelRevPosit}{.55}
\newcommand{\ArcLabelPosit}{.4}\newcommand{\ArcLabelRevPosit}{.6}
\newcommand{\LArcLabelPosit}{.4}\newcommand{\LArcLabelRevPosit}{.6}
\newcommand{\LoopLabelPosit}{.25}\newcommand{\LoopLabelRevPosit}{.75}
\newcommand{\CLoopLabelPosit}{.25}\newcommand{\CLoopLabelRevPosit}{.75}
% label position on initial-final arrow
\newcommand{\InitStateLabelPosit}{.1}
\newcommand{\InitStateLabelRevPosit}{.9}
\newcommand{\FinalStateLabelPosit}{.9}
\newcommand{\FinalStateLabelRevPosit}{.1}
%%% Size of initial and final arrow
% the size is relative to the diameter
% and the coefficient varies with the diameter
\newcommand{\ArrowOnStateCoef}{}
\newcommand{\ArrowOnMediumState}{1.5}
\newcommand{\ArrowOnSmallState}{1.7} 
\newcommand{\ArrowOnLargeState}{1.3}
\newcommand{\ArrowOnVerySmallState}{5} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Shift for aligned labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\VertShiftH} \settoheight{\VertShiftH}{$\{$}
\newlength{\VertShiftD} \settodepth{\VertShiftD}{$\{$}
\newlength{\VertShift}
\setlength{\VertShift}{.5\VertShiftD-.5\VertShiftH}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% flags 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\ifVCFrame
\newcommand{\HideFrame}{\VCFramefalse}
\newcommand{\ShowFrame}{\VCFrametrue}
\newif\ifVCGrid
\newcommand{\HideGrid}{\VCGridfalse}
\newcommand{\ShowGrid}{\VCGridtrue}
\newif\ifVCRigidLabel
\newcommand{\RigidLabel}{\VCRigidLabeltrue}
\newcommand{\SwivelLabel}{\VCRigidLabelfalse}
\newif\ifVCStateLabelBaseLine
\newcommand{\AlignedLabel}{\VCStateLabelBaseLinetrue}
\newcommand{\FloatingLabel}{\VCStateLabelBaseLinefalse}
\HideFrame
\HideGrid
\RigidLabel
\FloatingLabel
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   style for the frame around the picture
\psset{unit=1cm}
\newpsstyle{VaucFrameStyle}%
           {arrows=-,%
            framesep=0pt,%                   
            linewidth=0.6pt,%
            linecolor=black,%
            linestyle=solid,%
            doubleline=false,%
            fillcolor=white,%
            fillstyle=none,%
            cornersize=relative,%
            framearc=0}%
\newcommand{\FrameStyle}{\psset{style=VaucFrameStyle}}
\newpsstyle{VaucGridStyle}%
           {gridwidth=0.6pt,%
            griddots=10,%
            subgriddiv=1,%
            gridlabels=7pt}
\newcommand{\GridStyle}{\psset{style=VaucGridStyle}}
% figure, vertically centered by default
% draw frame according to VCFrame flag
% Set the shift for aligned label w.r.t the current size of characters
\newenvironment{VCPicture}[2][.5]%
   {\settoheight{\VertShiftH}{$\{$}%
    \settodepth{\VertShiftD}{$\{$}%
    \setlength{\VertShift}{.5\VertShiftD-.5\VertShiftH}%
    \begin{pspicture}[#1]#2%
       \ifVCFrame \FrameStyle \psframe#2\fi%
       \ifVCGrid \FrameStyle\GridStyle \psgrid#2\fi%
   }%
   {\RstState\RstEdge\end{pspicture}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scaling matters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% The "sizes" (for states) and the "line widths" are given 
%%% as "lengthes" in a fixed unit (cm or pt), whereas the positions 
%%% are supposed to be given in "psunits".
%%% This allows to use different scaling parameters 
%%% for the whole figure and for the "drawing grid".
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scaling commands
\newcommand{\VCScale}{0.6}% Global scale parameter
\newcommand{\VCGridScale}{1}% Global scale parameter
% 
\newcommand{\FixVCScale}[1]{\renewcommand{\VCScale}{#1}} 
\newcommand{\FixVCGridScale}[1]{\renewcommand{\VCGridScale}{#1}}
%                                              
\newcommand{\LargePicture}{\FixVCScale{\LargeScale}}
\newcommand{\MediumPicture}{\FixVCScale{\MediumScale}}
\newcommand{\SmallPicture}{\FixVCScale{\SmallScale}}
\newcommand{\TinyPicture}{\FixVCScale{\TinyScale}}
%%%%% Typical figure would look like
%   \scalebox{\VCScale}{%
%     \begin{VCPicture}{(x0,y0)(x1,y1)}
%     %  figure description
%     \end{VCPicture}%
%    }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Using a special directory for the figure
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\VCDirectory}{}
\newcommand{\SetVCDirectory}[1]{\renewcommand{\VCDirectory}{#1}}
% flag for printing the name of the figure file
\newif\ifVCName
\newcommand{\HideName}{\VCNamefalse}
\newcommand{\ShowName}{\VCNametrue}
\newcommand{\VCDraw}[2][\VCGridScale]%
   {\psset{unit=#1cm}%
    \scalebox{\VCScale}{#2}%
    \psset{unit=1cm}}
\newcommand{\VCCall}[2][\VCGridScale]%
   {\psset{unit=#1cm}%
    \ifVCName\makebox[0pt][r]{\fbox{{\scriptsize #2}}}\fi%
    \scalebox{\VCScale}{\input{\VCDirectory #2}}%
    \psset{unit=1cm}}
%%% commands
\newcommand{\VCPut}[3][0]{\rput{#1}#2{#3}}% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% State internal parameters  --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\StateLineWid}
\setlength{\StateLineWid}{\StateLineWidth}
\newcommand{\StateLineSty}{\StateLineStyle} 
\newcommand{\StateLineCol}{\StateLineColor}
%\newcommand{\StateLineDblSta}{\StateLineDblStatus}
\newcommand{\StateLineDblWid}{\StateLineDblWidth}
\newcommand{\StateLineDblSp}{\StateLineDblSep}
\newcommand{\StateFillCol}{\StateFillColor}
\newcommand{\StateFillSta}{\StateFillStatus} 
\newcommand{\StateLabelSca}{1}
\newcommand{\StateLabelCol}{\StateLabelColor}
\newcommand{\StateDimen}{outer}
\newcommand{\StateDblDimen}{middle}
%%%  Initial-final quality
\newcommand{\VCIFflag}{2}\newcommand{\VCIFflagtemp}{2}
\newcommand{\PlainState}%
  {\renewcommand{\VCIFflag}{0}\renewcommand{\VCIFflagtemp}{0}}
\newcommand{\FullState}%
  {\renewcommand{\VCIFflag}{2}\renewcommand{\VCIFflagtemp}{2}}
\newcommand{\IFState}{\renewcommand{\VCIFflag}{1}}
\newcommand{\IFXState}{\renewcommand{\VCIFflag}{2}}
\newcommand{\RstVCIF}{\renewcommand{\VCIFflag}{\VCIFflagtemp}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  State drawing style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% flag for hiding -- showing states (used for overlays in slides)
% the trick is to have two different styles and instead of 
% saving\restoring parameters
\newif\ifVCShowState
\newcommand{\HideState}{\VCShowStatefalse}
\newcommand{\ShowState}{\VCShowStatetrue}
\ShowState % initialisation
% the only difference between the two styles is the linestyle
\newpsstyle{VaucStateStyle}%
           {framesep=0pt,%                   
            linewidth=\StateLineWid,%
            linecolor=\StateLineCol,%
            linestyle=\StateLineSty,%
            doubleline=false,%
            fillcolor=\StateFillCol,%
            fillstyle=\StateFillSta,% 
            border=0pt,
            dimen=\StateDimen,%
            cornersize=relative,%
            framearc=1,%
            framesep=0pt}
\newpsstyle{VaucStateDblStyle}%
           {framesep=0pt,%                   
            linewidth=\StateLineDblCoef\StateLineWid,%
            linecolor=\StateLineCol,%
            linestyle=\StateLineSty,%
            doubleline=true,%
            doublesep=\StateLineDblSep\StateLineWid,%
            fillcolor=\StateFillCol,%
            fillstyle=\StateFillSta,% 
            border=0pt,%
            dimen=\StateDblDimen,%
            cornersize=relative,%
            framearc=1,%
            framesep=0pt}
\newpsstyle{VaucHiddenStateStyle}%
           {framesep=0pt,%                   
            linewidth=\StateLineWid,%
            linecolor=\StateLineCol,%
            linestyle=none,%
            fillcolor=\StateFillCol,%
            fillstyle=none,% 
            border=0pt,%
            dimen=outer,%
            cornersize=relative,%
            framearc=1,%
            framesep=0pt}
\newcommand{\StateStyle}%
   {\ifVCShowState%
       \ifStateLineDbl\psset{style=VaucStateDblStyle}%
       \else\psset{style=VaucStateStyle}%
       \fi%
    \else\psset{style=VaucHiddenStateStyle}%
    \fi}
%%% used in StateVar
\newcommand{\VaucStateRBLabel}[1]%
   {\textcolor{\StateLabelCol}%
              {\scalebox{\StateLabelSca}%
                        {\scalebox{\StateLabelScale}%
                                  {\rput[B]{0}(0,\VertShift){$#1$}}}}}
%%%
\newcommand{\VaucStateLabel}[1]%
    {\ifVCShowState%
        \ifVCRigidLabel%
           \ifVCStateLabelBaseLine%
              \textcolor{\StateLabelCol}%
                        {\scalebox{\StateLabelSca}%
                                  {\scalebox{\StateLabelScale}%
                                            {\rput[B]%
                                                  {*0}%
                                                  (0,\VertShift){$#1$}}}}%
           \else%
              \textcolor{\StateLabelCol}%
                        {\scalebox{\StateLabelSca}%
                                  {\scalebox{\StateLabelScale}%
                                            {\rput{*0}%
                                                  (0,0)%
                                                  {$ #1 $}}}}%
           \fi%
        \else%
           \textcolor{\StateLabelCol}%
                     {\scalebox{\StateLabelSca}%
                               {\scalebox{\StateLabelScale}{$#1$}}}%
        \fi%
     \else%
        \textcolor{white}%
                  {\scalebox{\StateLabelSca}
                            {\scalebox{\StateLabelScale}{$#1$}}}%
     \fi}
%%% Write label without state (not documented)
%%% 080612 new version that takes into account color, scale and 
%%% baseline
\newcommand{\VCStateLabel}[1]%
   {\ifVCStateLabelBaseLine
       \textcolor{\StateLabelCol}%
          {\scalebox{\StateLabelSca}%
             {\scalebox{\StateLabelScale}%
                {\rput[B]{0}(0,\VertShift){$#1$}}}}%
     \else
        \textcolor{\StateLabelCol}%
           {\scalebox{\StateLabelSca}%
              {\scalebox{\StateLabelScale}{$#1$}}}
     \fi
    }%
\newcommand{\VCPutStateLabel}[2]{\VCPut{#1}{\VCStateLabel{#2}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  State parameter changing and setting macros 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% line style
\newcommand{\ChgStateLineStyle}[1]{\renewcommand{\StateLineSty}{#1}}
\newcommand{\RstStateLineStyle}{\ChgStateLineStyle{\StateLineStyle}}
\newcommand{\SetStateLineStyle}[1]%
   {\renewcommand{\StateLineStyle}{#1}\RstStateLineStyle}%
%%% doubleline status
\newcommand{\StateLineDouble}{\StateLineDbltrue}
\newcommand{\StateLineSimple}{\StateLineDblfalse}
%%% line width
\newcommand{\ChgStateLineWidth}[1]%
   {\setlength{\StateLineWid}{#1\StateLineWidth}}%  
\newcommand{\RstStateLineWidth}{\ChgStateLineWidth{1}}%
\newcommand{\SetStateLineWidth}[1]% ATTN the parameter is a length
   {\setlength{\StateLineWidth}{#1}\RstStateLineWidth}
%%% line color
\newcommand{\ChgStateLineColor}[1]{\renewcommand{\StateLineCol}{#1}}
\newcommand{\RstStateLineColor}{\ChgStateLineColor{\StateLineColor}}
\newcommand{\SetStateLineColor}[1]%
   {\renewcommand{\StateLineColor}{#1}\RstStateLineColor}
%%% background fill status
\newcommand{\ChgStateFillStatus}[1]{\renewcommand{\StateFillSta}{#1}}
\newcommand{\RstStateFillStatus}{\ChgStateFillStatus{\StateFillStatus}}
\newcommand{\SetStateFillStatus}[1]% 
    {\renewcommand{\StateFillStatus}{#1}\RstStateFillStatus}
%%% backgroud color
\newcommand{\ChgStateFillColor}[1]{\renewcommand{\StateFillCol}{#1}}
\newcommand{\RstStateFillColor}{\ChgStateFillColor{\StateFillColor}}
\newcommand{\SetStateFillColor}[1]% 
    {\renewcommand{\StateFillColor}{#1}\RstStateFillColor}%
%%% label color
\newcommand{\ChgStateLabelColor}[1]{\renewcommand{\StateLabelCol}{#1}}
\newcommand{\RstStateLabelColor}{\ChgStateLabelColor{\StateLabelColor}}
\newcommand{\SetStateLabelColor}[1]%
    {\renewcommand{\StateLabelColor}{#1}\RstStateLabelColor}
%%% label scale
\newcommand{\ChgStateLabelScale}[1]{\renewcommand{\StateLabelSca}{#1}}
\newcommand{\RstStateLabelScale}{\ChgStateLabelScale{1}}
\newcommand{\SetStateLabelScale}[1]%
   {\renewcommand{\StateLabelScale}{#1}\RstStateLabelScale}
%%% double line
\newcommand{\FixStateLineDouble}[2]%
   {\renewcommand{\StateLineDblCoef}{#1}%
    \renewcommand{\StateLineDblSep}{#2}}
%%% dimmed state
\newcommand{\FixDimState}[5]%
   {\renewcommand{\DimStateLineStyle}{#1}%
    \renewcommand{\DimStateLineCoef}{#3}%
    \renewcommand{\DimStateLineColor}{#2}%
    \renewcommand{\DimStateLabelColor}{#4}%
    \renewcommand{\DimStateFillColor}{#5}}
\newcommand{\DimState}%
   {\ChgStateLineStyle{\DimStateLineStyle}%
    \ChgStateLineWidth{\DimStateLineCoef}%
    \ChgStateLineColor{\DimStateLineColor}%
    \ChgStateFillColor{\DimStateFillColor}%
    \ChgStateLabelColor{\DimStateLabelColor}}
%%% restoring state parameters
\newcommand{\RstState}%
   {\RstStateLineStyle%
    \RstStateLineWidth%
    \RstStateLineColor%
    \RstStateFillStatus%
    \RstStateFillColor%
    \RstStateLabelColor%
    \RstStateLabelScale}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% State drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% preparation
\newlength{\StateDiam}
\newlength{\VaucAOS}\newlength{\VaucAOSdiag}
%%%  A flag to remember the current size of state
\newcommand{\StateSizeFlag}{}
%
\newcommand{\SetAOS}%
   {\setlength{\VaucAOS}{\ArrowOnStateCoef\StateDiam}%
    \setlength{\VaucAOSdiag}{\SQRTwo\VaucAOS}}
%% parameter for variable width states
\newlength{\VariableStateIntDiam}
\newlength{\VariableStateWidth}
\newlength{\VariableStateITPos}
\newcommand{\SetStateIntDiam}%
   {\setlength{\VariableStateIntDiam}{\StateDiam}%
    \addtolength{\VariableStateIntDiam}{-2\StateLineWid}}
% Loop parameters
\newcommand{\LoopSize}{}\newcommand{\LoopSi}{}
\newcommand{\LoopVarSize}{}\newcommand{\LoopVarSi}{}
\newcommand{\CLoopSize}{}\newcommand{\CLoopSi}{}
%
\newcommand{\ChgLoopSize}[1]{\renewcommand{\LoopSi}{#1}}
\newcommand{\RstLoopSize}{\ChgLoopSize{\LoopSize}}
\newcommand{\SetLoopSize}[1]%
   {\renewcommand{\LoopSize}{#1}\RstLoopSize}
%
\newcommand{\ChgCLoopSize}[1]{\renewcommand{\CLoopSi}{#1}}
\newcommand{\RstCLoopSize}{\ChgCLoopSize{\CLoopSize}}
\newcommand{\SetCLoopSize}[1]%
   {\renewcommand{\CLoopSize}{#1}\RstCLoopSize}
%
\newcommand{\ChgLoopVarSize}[1]{\renewcommand{\LoopVarSi}{#1}}
\newcommand{\RstLoopVarSize}{\ChgLoopVarSize{\LoopVarSize}}
\newcommand{\SetLoopVarSize}[1]%
   {\renewcommand{\LoopVarSize}{#1}\RstLoopVarSize}
%
%%% setting state diameter -- internal command
\newcommand{\SetStateDiam}[4]%
   {\setlength{\StateDiam}{#1}%
    \renewcommand{\ArrowOnStateCoef}{#2}%
    \SetLoopSize{#3}%
    \SetLoopVarSize{#3}%
    \SetCLoopSize{#4}%
    \SetStateIntDiam%
    \SetAOS}
%%% setting state diameter -- external command
\newcommand{\FixStateDiameter}[1]%  
   {\setlength{\StateDiam}{#1}%
    \SetStateIntDiam%
    \SetAOS}
%%% setting coeff for initial/final arrows
\newcommand{\FixAOSLengthCoef}[1]%
   {\renewcommand{\ArrowOnStateCoef}{#1}%
    \SetAOS}
%%%
\newcommand{\MediumState}%
   {\SetStateDiam{\MediumStateDiameter}%
                 {\ArrowOnMediumState}%
                 {\LoopOnMediumState}%
                 {\CLoopOnMediumState}%
    \renewcommand{\StateSizeFlag}{0}}
\newcommand{\SmallState}%
   {\SetStateDiam{\SmallStateDiameter}%
                 {\ArrowOnSmallState}%
                 {\LoopOnSmallState}%
                 {\CLoopOnSmallState}%
    \renewcommand{\StateSizeFlag}{1}}
\newcommand{\LargeState}%
   {\SetStateDiam{\LargeStateDiameter}%
                 {\ArrowOnLargeState}%
                 {\LoopOnLargeState}
                 {\CLoopOnLargeState}%
    \renewcommand{\StateSizeFlag}{2}}
%
\newcommand{\RstStateSize}%
  {\ifthenelse{\equal{\StateSizeFlag}{0}}%
      {\MediumState}%
      {\ifthenelse{\equal{\StateSizeFlag}{1}}%
          {\SmallState}{\LargeState}}}
%%% Initialization
\MediumState
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\VaucState}[3][{}]%
   {\rput#2%
       {\Cnode[radius=.5\StateDiam](0,0){#3}%
        \ifVCShowState%
           \nput[labelsep=-.5\StateDiam]%
               {0}{#3}{\makebox[0pt]{\VaucStateLabel{#1}}}%
        \fi%
        \ifthenelse{\equal{\VCIFflag}{0}}%
           {}%
           {\pnode(-\VaucAOS,0){#3w}%
            \pnode(\VaucAOS,0){#3e}%
            \pnode(0,\VaucAOS){#3n}%
            \pnode(0,-\VaucAOS){#3s}%
            \ifthenelse{\equal{\VCIFflag}{1}}%
               {}%
               {\pnode(-\VaucAOSdiag,\VaucAOSdiag){#3nw}%
                \pnode(\VaucAOSdiag,\VaucAOSdiag){#3ne}%
                \pnode(-\VaucAOSdiag,-\VaucAOSdiag){#3sw}%
                \pnode(\VaucAOSdiag,-\VaucAOSdiag){#3se}}%
           }%
       }%
   }
%
\newcommand{\State}[3][{}]{\StateStyle\VaucState[#1]{#2}{#3}}
%
\newcommand{\FinalState}[3][{}]%
   {\psset{style=VaucStateDblStyle}%
    \VaucState[#1]{#2}{#3}}
%%% ecological commands   
\newcommand{\StateIF}[3][{}]{\IFState\State[#1]{#2}{#3}\RstVCIF}%
\newcommand{\StateIFX}[3][{}]{\IFXState\State[#1]{#2}{#3}\RstVCIF}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Very Small State   
\newcommand{\VSState}[2]%
    {\renewcommand{\ArrowOnStateCoef}{\ArrowOnVerySmallState}%
     \FixStateDiameter{\VerySmallStateDiameter}%
     \ChgStateLineWidth{\VSStateLineCoef}%
     \State{#1}{#2}%
     \RstStateLineWidth%
     \RstStateSize}% mod 020201
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% white brace, of no width, used to place the label vertically
%\newlength{\BraceLength}
\newcommand{\WB}{\textcolor{white}{\{\!\!\!}}%
\newcommand{\HS}{}
\newlength{\ExtraSpace}\setlength{\ExtraSpace}{1em}
%
\newcommand{\StateVar}[3][]%
   {\StateStyle%
    \settowidth{\VariableStateWidth}%
               {\scalebox{\StateLabelSca}%
                         {\scalebox{\StateLabelScale}{$#1$}}}%
    \addtolength{\VariableStateWidth}{\ExtraSpace}%
    \ifthenelse{\lengthtest{\VariableStateWidth<\VariableStateIntDiam}}%
       {\setlength{\VariableStateWidth}{\VariableStateIntDiam}}%
       {}%
    \setlength{\VariableStateITPos}{\ArrowOnStateCoef\StateDiam}%
    \addtolength{\VariableStateITPos}{0.5\VariableStateWidth}%
    \addtolength{\VariableStateITPos}{-0.5\StateDiam}%
    \rput#2%
       {\pnode(\VariableStateITPos,0){#3e}%
        \pnode(-\VariableStateITPos,0){#3w}%
        \pnode(0,\ArrowOnStateCoef\StateDiam){#3n}%
        \pnode(0,-\ArrowOnStateCoef\StateDiam){#3s}}%
    \rput#2%
       {\rnode{#3}%
              {\psframebox{\protect\rule[-.5\VariableStateIntDiam]%
                                        {0pt}%
                                        {\VariableStateIntDiam}%                                           
                           \protect\rule{\VariableStateWidth}{0pt}}}}%
    \rput#2{\VaucStateRBLabel{#1}}%
   }%
%%%%% macro FinalStateVar %%%%%%%%%%%%%%%%%%%
\newcommand{\StateLineDblTemp}{0}
\newcommand{\FinalStateVar}[3][]%
   {\ifStateLineDbl\renewcommand{\StateLineDblTemp}{1}%
    \else\renewcommand{\StateLineDblTemp}{0}%
    \fi%
    \StateLineDouble%
    \StateVar[#1]{#2}{#3}%
    \ifthenelse{\equal{\StateLineDblTemp}{0}}%
       {\StateLineSimple}{}%
    }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\VarLoopOn}%
   {\ChgLoopOffset{\LoopVarOff}%
    \ChgLoopSize{\LoopVarSi}%
    \ChgLoopAngle{\LoopVarAng}}
\newcommand{\VarLoopOff}{\RstLoopOffset\RstLoopSize\RstLoopAngle}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge drawing parameters  --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\EdgeLineWid}
\setlength{\EdgeLineWid}{\EdgeLineWidth}
\newcommand{\EdgeLineSty}{\EdgeLineStyle}
\newcommand{\EdgeLineCol}{\EdgeLineColor}
% label
\newcommand{\EdgeLabelSca}{1}
\newcommand{\EdgeLabelCol}{\EdgeLabelColor}
% arrow
\newlength{\EdgeArrowSZDim}
\setlength{\EdgeArrowSZDim}{\EdgeArrowWidth}
\newcommand{\EdgeArrowSZNum}{\EdgeArrowLengthCoef}
\newcommand{\EdgeArrowSty}{\EdgeArrowStyle}
\newcommand{\EdgeArrowIns}{\EdgeArrowInset}
% border 
\newlength{\EdgeLineBord}\setlength{\EdgeLineBord}{0pt}
%%% Zigzag edge parameters
\newlength{\ZZSiZ}
\setlength{\ZZSiZ}{\ZZSize}%
\newcommand{\ZZLineWid}{\ZZLineWidth}% multiplying coefficient
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge geometric parameters  --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Edge 
\newlength{\EdgeOff}
\setlength{\EdgeOff}{\EdgeOffset}
% Arc
\newcommand{\VaucArcAng}{\VaucArcAngle}
\newcommand{\VaucLArcAng}{\VaucLArcAngle}
\newlength{\VaucArcOff}
\setlength{\VaucArcOff}{\VaucArcOffset}
% Loop
\newcommand{\VaucArcCurv}{\VaucArcCurvature}
\newcommand{\VaucLArcCurv}{\VaucLArcCurvature}
\newcommand{\LoopAng}{\LoopAngle}
\newcommand{\CLoopAng}{\CLoopAngle}
\newcommand{\LoopVarAng}{\LoopVarAngle}
\newlength{\LoopOff}\setlength{\LoopOff}{\LoopOffset}
\newlength{\LoopVarOff}\setlength{\LoopVarOff}{\LoopVarOffset}
\newlength{\EdgeNodeSP}\setlength{\EdgeNodeSP}{\EdgeNodeSep}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Edge label parameters --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% label distance from transition
\newlength{\TransLabelSP}\setlength{\TransLabelSP}{\TransLabelSep}
% label position on transitions
\newcommand{\EdgeLabelPos}{\EdgeLabelPosit}
\newcommand{\ArcLabelPos}{\ArcLabelPosit}
\newcommand{\LArcLabelPos}{\LArcLabelPosit}
\newcommand{\LoopLabelPos}{\LoopLabelPosit}
\newcommand{\CLoopLabelPos}{\CLoopLabelPosit}
% label position on initial-final arrow
\newcommand{\InitStateLabelPos}{\InitStateLabelPosit}
\newcommand{\FinalStateLabelPos}{\FinalStateLabelPosit}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Transition styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpsstyle{VaucEdgeStyle}%
           {arrows=\EdgeArrowSty,%
            arrowsize=\EdgeArrowSZDim,%
            arrowlength=\EdgeArrowSZNum,%
            arrowinset=\EdgeArrowIns,%
            linewidth=\EdgeLineWid,%
            linecolor=\EdgeLineCol,%
            linestyle=\EdgeLineSty,%
            doubleline=false,%
            bordercolor=\EdgeLineBorderColor,%
            border=\EdgeLineBord,%
            fillstyle=none,%
            offset=\EdgeOff,%
            labelsep=\TransLabelSP,%
            nodesep=\EdgeNodeSP}
\newpsstyle{VaucEdgeDblStyle}%
           {arrows=\EdgeArrowSty,%
            arrowsize=\EdgeArrowSZDim,%
            arrowlength=\EdgeArrowSZNum,%
            arrowinset=\EdgeArrowIns,%
            linewidth=\EdgeLineDblCoef\EdgeLineWid,%
            linecolor=\EdgeLineCol,
            linestyle=\EdgeLineSty,%
            doubleline=true,%
            doublesep=\EdgeLineDblSep\EdgeLineWid,%
            bordercolor=\EdgeLineBorderColor,%
            border=\EdgeLineBord,%
            fillstyle=none,%
            offset=\EdgeOff,%
            labelsep=\TransLabelSP,%
            nodesep=\EdgeNodeSP}
%%% Arc
\newpsstyle{VaucArcR}%
           {ncurv=\VaucArcCurv,%
            arcangle=-\VaucArcAng,%
            labelsep=\TransLabelSP,%
            offset=-\VaucArcOff}
\newpsstyle{VaucArcL}%
           {ncurv=\VaucArcCurv,%
            arcangle=\VaucArcAng,%
            labelsep=\TransLabelSP,%
            offset=\VaucArcOff}
\newpsstyle{VaucLArcR}%
           {ncurv=\VaucLArcCurv,%
            arcangle=-\VaucLArcAng,%
            labelsep=\TransLabelSP,%
            offset=-\VaucArcOff}
\newpsstyle{VaucLArcL}%
           {ncurv=\VaucLArcCurv,%
            arcangle=\VaucLArcAng,%
            labelsep=\TransLabelSP,%
            offset=\VaucArcOff}
%%% zig-zag
\newpsstyle{VaucZigzagStyle}%
           {linewidth=\ZZLineWid\EdgeLineWid,%
            linearc=1.6pt,%
            coilwidth=1.2\ZZSiZ,%
            coilheight=\ZZShape,%
            coilarmA=0.1\ZZSiZ,%
            coilarmB=0.3\ZZSiZ,%
            labelsep=\TransLabelSP,%
            nodesep=\EdgeNodeSP}
%%%
\newcommand{\EdgeStyle}%
   {\ifEdgeLineDbl\psset{style=VaucEdgeDblStyle}%
    \else\psset{style=VaucEdgeStyle}%
    \fi}
\newcommand{\ZigzagStyle}%
   {\addtolength{\TransLabelSP}{\TransLabelZZCoef\ZZSiZ}%
    \psset{style=VaucZigzagStyle}%
    \addtolength{\TransLabelSP}{-\TransLabelZZCoef\ZZSiZ}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Transition parameter changing and setting macros 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% geometric parameters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  edges
\newcommand{\ChgEdgeOffset}[1]{\setlength{\EdgeOff}{#1}}
\newcommand{\RstEdgeOffset}{\ChgEdgeOffset{\EdgeOffset}}
\newcommand{\SetEdgeOffset}[1]%
   {\setlength{\EdgeOffset}{#1}\RstEdgeOffset}
\newcommand{\ForthBackOffset}%
   {\setlength{\EdgeOff}{\ForthBackEdgeOffset\EdgeLineWid}}
%
\newcommand{\ChgEdgeNodeSep}[1]{\setlength{\EdgeNodeSP}{#1\EdgeNodeSep}}
\newcommand{\RstEdgeNodeSep}{\ChgEdgeNodeSep{1}}
\newcommand{\SetEdgeNodeSep}[1]%
   {\setlength{\EdgeNodeSep}{#1}\RstEdgeNodeSep}
%%  arcs
\newcommand{\ChgArcAngle}[1]{\renewcommand{\VaucArcAng}{#1}}
\newcommand{\RstArcAngle}{\ChgArcAngle{\VaucArcAngle}}
\newcommand{\SetArcAngle}[1]%
   {\renewcommand{\VaucArcAngle}{#1}\RstArcAngle}
%
\newcommand{\ChgLArcAngle}[1]{\renewcommand{\VaucLArcAng}{#1}}
\newcommand{\RstLArcAngle}{\ChgLArcAngle{\VaucLArcAngle}}
\newcommand{\SetLArcAngle}[1]%
   {\renewcommand{\VaucLArcAngle}{#1}\RstLArcAngle}
%
\newcommand{\ChgArcCurvature}[1]{\renewcommand{\VaucArcCurv}{#1}}
\newcommand{\RstArcCurvature}{\ChgArcCurvature{\VaucArcCurvature}}
\newcommand{\SetArcCurvature}[1]%
   {\renewcommand{\VaucArcCurvature}{#1}\RstArcCurvature}
%
\newcommand{\ChgLArcCurvature}[1]{\renewcommand{\VaucLArcCurv}{#1}}
\newcommand{\RstLArcCurvature}{\ChgLArcCurvature{\VaucLArcCurvature}}
\newcommand{\SetLArcCurvature}[1]%
   {\renewcommand{\VaucLArcCurvature}{#1}\RstLArcCurvature}
%
\newcommand{\ChgArcOffset}[1]{\setlength{\VaucArcOff}{#1}}
\newcommand{\RstArcOffset}{\setlength{\VaucArcOff}{\VaucArcOffset}}
\newcommand{\SetArcOffset}[1]%
   {\renewcommand{\VaucArcOffset}{#1}\RstArcOffset}
%
\newcommand{\ChgLoopOffset}[1]{\setlength{\LoopOff}{#1}}
\newcommand{\RstLoopOffset}{\setlength{\LoopOff}{\LoopOffset}}
\newcommand{\SetLoopOffset}[1]%
   {\renewcommand{\LoopOffset}{#1}\RstLoopOffset}
%
\newcommand{\ChgLoopAngle}[1]{\renewcommand{\LoopAng}{#1}}
\newcommand{\RstLoopAngle}{\ChgLoopAngle{\LoopAngle}}
\newcommand{\SetLoopAngle}[1]%
   {\renewcommand{\LoopAngle}{#1}\RstLoopAngle}
%
\newcommand{\ChgCLoopAngle}[1]{\renewcommand{\CLoopAng}{#1}}
\newcommand{\RstCLoopAngle}{\ChgCLoopAngle{\CLoopAngle}}
\newcommand{\SetCLoopAngle}[1]%
   {\renewcommand{\CLoopAngle}{#1}\RstCLoopAngle}
%%  labels
\newcommand{\ChgEdgeLabelSep}[1]%
   {\setlength{\TransLabelSP}{#1\TransLabelSep}}
\newcommand{\RstEdgeLabelSep}{\ChgEdgeLabelSep{1}}
\newcommand{\SetEdgeLabelSep}[1]%
   {\setlength{\TransLabelSep}{#1}\RstEdgeLabelSep}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% drawing parameters
\newcommand{\ChgEdgeLineColor}[1]{\renewcommand{\EdgeLineCol}{#1}}
\newcommand{\RstEdgeLineColor}{\ChgEdgeLineColor{\EdgeLineColor}}
\newcommand{\SetEdgeLineColor}[1]%
   {\renewcommand{\EdgeLineColor}{#1}\RstEdgeLineColor}
%
\newcommand{\ChgEdgeLineStyle}[1]{\renewcommand{\EdgeLineSty}{#1}}  
\newcommand{\RstEdgeLineStyle}{\ChgEdgeLineStyle{\EdgeLineStyle}}
\newcommand{\SetEdgeLineStyle}[1]%
   {\renewcommand{\EdgeLineStyle}{#1}\RstEdgeLineStyle}
%
\newcommand{\ChgEdgeLineWidth}[1]% coefficient !
   {\setlength{\EdgeLineWid}{#1\EdgeLineWidth}}
\newcommand{\RstEdgeLineWidth}{\ChgEdgeLineWidth{1}}
\newcommand{\SetEdgeLineWidth}[1]% length !
   {\setlength{\EdgeLineWidth}{#1}\RstEdgeLineWidth}
% double line
\newcommand{\EdgeLineDouble}%
   {\EdgeLineDbltrue%
    \ChgEdgeArrowWidth{\EdgeDblArrowWidth}%
    \ChgEdgeArrowLengthCoef{\EdgeDblArrowLengthCoef}}
\newcommand{\EdgeLineSimple}%
   {\EdgeLineDblfalse\RstEdgeArrowWidth\RstEdgeArrowLengthCoef}
\newcommand{\FixEdgeLineDouble}[2]{%
    \renewcommand{\EdgeLineDblCoef}{#1}%
    \renewcommand{\EdgeLineDblSep}{#2}}
% edge labels
\newcommand{\ChgEdgeLabelColor}[1]{\renewcommand{\EdgeLabelCol}{#1}}
\newcommand{\RstEdgeLabelColor}{\ChgEdgeLabelColor{\EdgeLabelColor}}
\newcommand{\SetEdgeLabelColor}[1]%
   {\renewcommand{\EdgeLabelColor}{#1}\RstEdgeLabelColor}
%
\newcommand{\ChgEdgeLabelScale}[1]{\renewcommand{\EdgeLabelSca}{#1}}
\newcommand{\RstEdgeLabelScale}{\ChgEdgeLabelScale{1}}
\newcommand{\SetEdgeLabelScale}[1]%
   {\renewcommand{\EdgeLabelScale}{#1}\RstEdgeLabelScale}
% arrows
\newcommand{\ChgEdgeArrowStyle}[1]{\renewcommand{\EdgeArrowSty}{#1}}
\newcommand{\RstEdgeArrowStyle}{\ChgEdgeArrowStyle{\EdgeArrowStyle}}
\newcommand{\SetEdgeArrowStyle}[1]%
   {\renewcommand{\EdgeArrowStyle}{#1}\RstEdgeArrowStyle}
%
\newcommand{\ChgEdgeArrowWidth}[1]%
   {\setlength{\EdgeArrowSZDim}{#1}} % !! length !!
\newcommand{\RstEdgeArrowWidth}{\ChgEdgeArrowWidth{\EdgeArrowWidth}}
\newcommand{\SetEdgeArrowWidth}[1]%
   {\setlength{\EdgeArrowWidth}{#1} \RstEdgeArrowWidth}
%
\newcommand{\ChgEdgeArrowLengthCoef}[1]{\renewcommand{\EdgeArrowSZNum}{#1}}
\newcommand{\RstEdgeArrowLengthCoef}{\ChgEdgeArrowLengthCoef{\EdgeArrowLengthCoef}}
\newcommand{\SetEdgeArrowLengthCoef}[1]%
   {\renewcommand{\EdgeArrowLengthCoef}{#1}\RstEdgeArrowLengthCoef}
%
\newcommand{\ChgEdgeArrowInsetCoef}[1]{\renewcommand{\EdgeArrowIns}{#1}}
\newcommand{\RstEdgeArrowInsetCoef}{\ChgEdgeArrowInsetCoef{\EdgeArrowInset}}
\newcommand{\SetEdgeArrowInsetCoef}[1]%
   {\renewcommand{\EdgeArrowInset}{#1}\RstEdgeArrowInsetCoef}
%
\newcommand{\ReverseArrow}%
   {\ChgEdgeArrowStyle{\EdgeRevArrowStyle}%
    \renewcommand{\EdgeLabelPos}{\EdgeLabelRevPosit}%
    \renewcommand{\ArcLabelPos}{\ArcLabelRevPosit}%
    \renewcommand{\LArcLabelPos}{\LArcLabelRevPosit}%
    \renewcommand{\LoopLabelPos}{\LoopLabelRevPosit}%
    \renewcommand{\CLoopLabelPos}{\CLoopLabelRevPosit}%
    \renewcommand{\InitStateLabelPos}{\InitStateLabelRevPosit}%
    \renewcommand{\FinalStateLabelPos}{\FinalStateLabelRevPosit}}
\newcommand{\StraightArrow}%
   {\ChgEdgeArrowStyle{\EdgeArrowStyle}%
    \renewcommand{\EdgeLabelPos}{\EdgeLabelPosit}%
    \renewcommand{\ArcLabelPos}{\ArcLabelPosit}%
    \renewcommand{\LArcLabelPos}{\LArcLabelPosit}%
    \renewcommand{\LoopLabelPos}{\LoopLabelPosit}%
    \renewcommand{\CLoopLabelPos}{\CLoopLabelPosit}%
    \renewcommand{\InitStateLabelPos}{\InitStateLabelPosit}%
    \renewcommand{\FinalStateLabelPos}{\FinalStateLabelPosit}}
% border
\newcommand{\FixEdgeBorder}[2]%
   {\renewcommand{\EdgeLineBorderCoef}{#1}%
    \renewcommand{\EdgeLineBorderColor}{#2}}
\newcommand{\EdgeBorder}%
  {\setlength{\EdgeLineBord}{\EdgeLineBorderCoef\EdgeLineWid}}
\newcommand{\EdgeBorderOff}{\setlength{\EdgeLineBord}{0pt}}
% dimmed edges
\newcommand{\FixDimEdge}[4]{%
    \renewcommand{\DimEdgeLineStyle}{#1}%
    \renewcommand{\DimEdgeLineCoef}{#2}%
    \renewcommand{\DimEdgeLineColor}{#3}%
    \renewcommand{\DimEdgeLabelColor}{#4}}%
%
\newcommand{\DimEdge}%
   {\ChgEdgeLineStyle{\DimEdgeLineStyle}%
    \ChgEdgeLineWidth{\DimEdgeLineCoef}%
    \ChgEdgeLineColor{\DimEdgeLineColor}%
    \ChgEdgeLabelColor{\DimEdgeLabelColor}}
% zigzag edges
\newcommand{\ChgZZSize}[1]{\setlength{\ZZSiZ}{#1}}
\newcommand{\RstZZSize}{\setlength{\ZZSiZ}{\ZZSize}}
\newcommand{\SetZZSize}[1]{\setlength{\ZZSiZe}{#1}\RstZZSize}
%
\newcommand{\ChgZZLineWidth}[1]{\renewcommand{\ZZLineWid}{#1}}
\newcommand{\RstZZLineWidth}{\ChgZZLineWidth{\ZZLineWidth}}
\newcommand{\SetZZLineWidth}[1]%
   {\renewcommand{\ZZLineWidth}{#1}\RstZZLineWidth}
%%%
\newcommand{\RstEdge}%
   {\RstEdgeOffset%
    \RstArcAngle%
    \RstLArcAngle%
    \RstArcCurvature%
    \RstLArcCurvature%
    \RstArcOffset%
    \RstLoopOffset%
    \RstLoopSize%
    \RstEdgeLineColor%
    \RstEdgeLineStyle%
    \RstEdgeLineWidth%
    \EdgeLineSimple%
    \StraightArrow%\EdgeBorderOff%
    \RstEdgeLabelScale%
    \RstEdgeLabelColor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Transition drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% composition of transition label 
\newcommand{\VaucEdgeLabel}[1]%
   {\textcolor{\EdgeLabelCol}%
              {\scalebox{\EdgeLabelSca}%
                        {\scalebox{\EdgeLabelScale}{$#1$}}}}% 
%%% Edges
\newcommand{\EdgeL}[4][{\EdgeLabelPos}]%
   {\EdgeStyle \ncline{#2}{#3} \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\EdgeR}[4][{\EdgeLabelPos}]%
   {\EdgeStyle \ncline{#2}{#3} \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%%% Arcs 
\newcommand{\ArcL}[4][{\ArcLabelPos}]%
   {\EdgeStyle%
    \psset{style=VaucArcL}% 
    \ncarc{#2}{#3}%
    \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\ArcR}[4][{\ArcLabelPos}]%
   {\EdgeStyle%
    \psset{style=VaucArcR}% 
    \ncarc{#2}{#3}%
    \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\LArcL}[4][{\LArcLabelPos}]%
   {\EdgeStyle%
    \psset{style=VaucLArcL}% 
    \ncarc{#2}{#3}%
    \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\LArcR}[4][{\LArcLabelPos}]%
   {\EdgeStyle%
    \psset{style=VaucLArcR}% 
    \ncarc{#2}{#3}%
    \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%%% Loops
\newcounter{anglea}\newcounter{angleb}
\newcommand{\LoopXR}[7]%
   {{\setcounter{anglea}{#2-#4}}%
    {\setcounter{angleb}{#2+#4}}%
    {\EdgeStyle%
     \psset{angleA=\theanglea,angleB=\theangleb,offset=#5,ncurv=#6}% 
     \nccurve{#3}{#3}%
     \nbput[npos=#1]{\VaucEdgeLabel{#7}}}}
\newcommand{\LoopXL}[7]%
   {{\setcounter{anglea}{#2+#4}}%
    {\setcounter{angleb}{#2-#4}}%
    {\EdgeStyle%
     \psset{angleA=\theanglea,angleB=\theangleb,offset=-#5,ncurv=#6}% 
     \nccurve{#3}{#3}%
     \naput[npos=#1]{\VaucEdgeLabel{#7}}}}
%
\newcommand{\LoopR}[4][{\LoopLabelPos}]%
   {\LoopXR{#1}{#2}{#3}{\LoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\LoopL}[4][{\LoopLabelPos}]%
   {\LoopXL{#1}{#2}{#3}{\LoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\CLoopR}[4][{\CLoopLabelPos}]%
   {\LoopXR{#1}{#2}{#3}{\CLoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\CLoopL}[4][{\CLoopLabelPos}]%
   {\LoopXL{#1}{#2}{#3}{\CLoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\LoopVarR}[4][{\LoopLabelPos}]%
   {\LoopXR{#1}{#2}{#3}{\LoopVarAng}{\LoopVarOff}{\LoopVarSi}{#4}}
\newcommand{\LoopVarL}[4][{\LoopLabelPos}]%
   {\LoopXL{#1}{#2}{#3}{\LoopVarAng}{\LoopVarOff}{\LoopVarSi}{#4}}
%
\newcommand{\LoopW}[3][{\LoopLabelPos}]{\LoopR[#1]{180}{#2}{#3}}
\newcommand{\LoopE}[3][{\LoopLabelPos}]{\LoopL[#1]{0}{#2}{#3}}
\newcommand{\LoopN}[3][{\LoopLabelPos}]{\LoopL[#1]{90}{#2}{#3}}
\newcommand{\LoopS}[3][{\LoopLabelPos}]{\LoopR[#1]{-90}{#2}{#3}}
\newcommand{\LoopNW}[3][{\LoopLabelPos}]{\LoopR[#1]{135}{#2}{#3}}
\newcommand{\LoopNE}[3][{\LoopLabelPos}]{\LoopL[#1]{45}{#2}{#3}}
\newcommand{\LoopSW}[3][{\LoopLabelPos}]{\LoopL[#1]{-135}{#2}{#3}}
\newcommand{\LoopSE}[3][{\LoopLabelPos}]{\LoopR[#1]{-45}{#2}{#3}}
\newcommand{\CLoopW}[3][{\CLoopLabelPos}]{\CLoopR[#1]{180}{#2}{#3}}
\newcommand{\CLoopE}[3][{\CLoopLabelPos}]{\CLoopL[#1]{0}{#2}{#3}}
\newcommand{\CLoopN}[3][{\CLoopLabelPos}]{\CLoopL[#1]{90}{#2}{#3}}
\newcommand{\CLoopS}[3][{\CLoopLabelPos}]{\CLoopR[#1]{-90}{#2}{#3}}
\newcommand{\CLoopNW}[3][{\CLoopLabelPos}]{\CLoopR[#1]{135}{#2}{#3}}
\newcommand{\CLoopNE}[3][{\CLoopLabelPos}]{\CLoopL[#1]{45}{#2}{#3}}
\newcommand{\CLoopSW}[3][{\CLoopLabelPos}]{\CLoopL[#1]{-135}{#2}{#3}}
\newcommand{\CLoopSE}[3][{\CLoopLabelPos}]{\CLoopR[#1]{-45}{#2}{#3}}
\newcommand{\LoopVarN}[3][{\CLoopLabelPos}]{\LoopVarL[#1]{90}{#2}{#3}}
\newcommand{\LoopVarS}[3][{\CLoopLabelPos}]{\LoopVarR[#1]{-90}{#2}{#3}}
%%% Zigzag edges
\newcommand{\ZZEdge}[2]%
   {\EdgeStyle%
    \ZigzagStyle%
    \nczigzag{#1}{#2}}
\newcommand{\ZZEdgeL}[4][{\EdgeLabelRevPosit}]%
   {\EdgeStyle%
    \ZigzagStyle%
    \nczigzag{#2}{#3}%
    \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\ZZEdgeR}[4][{\EdgeLabelRevPosit}]%
   {\EdgeStyle%
    \ZigzagStyle%
    \nczigzag{#2}{#3}%
    \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Initial-final arrow drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% implicit parameter
\newcommand{\InitialDir}{w}\newcommand{\FinalDir}{e}
% without label
\newcommand{\Initial}[2][\InitialDir]{\EdgeStyle\ncline{#2#1}{#2}}
\newcommand{\Final}[2][\FinalDir]{\EdgeStyle\ncline{#2}{#2#1}}
% with label
%  NB modified syntax eg \InitialL[pos]{dir}{statename}{label}
\newcommand{\InitialL}[4][{\InitStateLabelPos}]%
   {\EdgeStyle%
    \ncline{#3#2}{#3}%
    \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\InitialR}[4][{\InitStateLabelPos}]%
   {\EdgeStyle%
    \ncline{#3#2}{#3}%
    \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\FinalL}[4][{\FinalStateLabelPos}]%
   {\EdgeStyle%
    \ncline{#3}{#3#2}%
    \naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\FinalR}[4][{\FinalStateLabelPos}]%
   {\EdgeStyle%
    \ncline{#3}{#3#2}%
    \nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Reprise des macros pstricks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Point}[2]{\pnode#1{#2}}
\newcommand{\Edge}[2]{\EdgeStyle\ncline{#1}{#2}}
%
\newcommand{\VArcL}[5][{\ArcLabelPos}]%
   {\EdgeStyle%
    \psset{style=VaucLArcL}% 
    \ncarc[#2]{#3}{#4}%
    \naput[npos=#1]{\VaucEdgeLabel{#5}}}
\newcommand{\VArcR}[5][{\ArcLabelPos}]%
   {\EdgeStyle%
    \psset{style=VaucLArcR}% 
    \ncarc[#2]{#3}{#4}%
    \nbput[npos=#1]{\VaucEdgeLabel{#5}}}
%
\newcommand{\VCurveL}[5][{\ArcLabelPos}]%
   {\EdgeStyle%
    \psset{angleA=0,angleB=180,ncurv=1}% 
    \nccurve[#2]{#3}{#4}%
    \naput[npos=#1]{\VaucEdgeLabel{#5}}}
\newcommand{\VCurveR}[5][{\ArcLabelPos}]%
   {\EdgeStyle%
    \psset{angleA=0,angleB=0,ncurv=1}% 
    \nccurve[#2]{#3}{#4}%
    \nbput[npos=#1]{\VaucEdgeLabel{#5}}}
%
\newcommand{\LabelL}[2][{\EdgeLabelPos}]%
   {\naput[npos=#1]{\VaucEdgeLabel{#2}}}
\newcommand{\LabelR}[2][{\EdgeLabelPos}]%
   {\nbput[npos=#1]{\VaucEdgeLabel{#2}}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> eptcsdata.tex <==
\providecommand{\firstpage}{49}
\providecommand{\publicationstatus}{M.R. Mousavi and A. Ravara: FOCLASA 2011\\
EPTCS 58, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.58.4}{10.4204/EPTCS.58.4}}

